Intraoperative Registration by Cross-Modal Inverse Neural Rendering

We present in this paper a novel approach for 3D/2D intraoperative registration during neurosurgery via cross-modal inverse neural rendering. Our approach separates implicit neural representation into two components, handling anatomical structure preoperatively and appearance intraoperatively. This disentanglement is achieved by controlling a Neural Radiance Field's appearance with a multi-style hypernetwork. Once trained, the implicit neural representation serves as a differentiable rendering engine, which can be used to estimate the surgical camera pose by minimizing the dissimilarity between its rendered images and the target intraoperative image. We tested our method on retrospective patients' data from clinical cases, showing that our method outperforms state-of-the-art while meeting current clinical standards for registration. Code and additional resources can be found at https://maxfehrentz.github.io/style-ngp/.

==> method-bis.tex <==
\begin{figure}[ht!]
     \begin{center}
%\begin{tabular}{c}
        \includegraphics[width=1\linewidth]{figs/pipeline.pdf}
%    \end{tabular}
    \end{center}
    \caption{Left (preoperative): We use a NeRF to first learn density/anatomy from a mesh $\mathbf{M}$ extracted from an MR scan (orange), then learn single-shot style adaptation through a hypernetwork $h$ while keeping the previously learned density $f_d$ (blue). Right (intraoperative): The method performs iterative pose estimation on a given target from the surgical microscope $\mathbf{I}$. The preoperatively trained NeRF and hypernet (green highlights) are used as style-conditioned neural rendering engine $f$ using ray casting, style-adapted on the intraoperative registration target $\mathbf{I}$ through the hypernetwork $h$.}
    \label{fig:overview}
\end{figure} 

\section{Methods}
%\begin{itemize}
%    \item TODO: fix/redo pipeline
%    \item TODO: change notations of super- and subscript
%    \item TODO: be consistent and pick: $t_{vr}$, $tex_{vr}$, and $t_\text{VR}$
%    \item TODO: be consistent with image names: $I$ for intraop, $J$ (with subscript) for all others?
%    \item TODO: be consistent with $F_c$, $F_{rgb}$, $F_{d}$, $F_{density}$
%    \item TODO: write rendering engine as $R$ and explain differently
%\end{itemize}
\subsection{Problem Formulation \& Overview}
% \begin{itemize}
%   \item Given: Intraoperative image from surgical microscope $I_{intraop}$ and surface mesh of the craniotomy area from preoperative scan (e.g. MRI) $M$, textured with volume rendering appearance $tex_{vr}$
%   \item Find: $\hat{P}$
%   \item Such that: $\hat{P} = \underset{P \in SE(3)}{\mathrm{argmin}} \; \mathcal{L}(P| I, M)$
%   \item In practice: 2D image space optimization problem
%   \item Our method: minimize image-based loss between $I$ and images rendered from a continuous, differentiable neural representation $F$
%   \item its structure is learned from $M$ preoperatively and its style is conditioned on $I$ intraoperatively
%   \item Solves 3D-to-2D dimensionality problem -> $F$ can render 2D images from anatomy learned from $M$
%   \item Crosses modality gap to $I$ with intraoperative style conditioning
%   \item reformulation for our method: $\hat{P} = \underset{P \in SE(3)}{\mathrm{argmin}} \; \mathcal{L}(I, F(P | I, M))$
%   \item Since $F$ is differentiable back to the camera pose, we can solve the equation by iteratively rendering a pose, computing an image-based loss and gradient w.r.t to $I$, updating the camera pose, ...
% \end{itemize}

% Given a preoperative surface mesh $M$ of the craniotomy area and an intraoperative image $I_{\text{intraop}}$ obtained from a surgical microscope, we seek to determine the pose $\hat{P}$ within the special Euclidean group $SE(3)$ that minimizes a loss function $\mathcal{L}$ which quantifies the discrepancy between the observed intraoperative image and preoperative mesh $M$ when positioned and oriented according to the pose $P$.
Given a preoperative surface mesh $\mathbf{M}$ of the craniotomy area and an intraoperative image $\mathbf{I}$ obtained from a surgical microscope, we seek to determine the pose $\mathbf{P} \in SE(3)$, where $SE(3)$ in the special Euclidean group $SE(3)$. This pose minimizes a loss function $\mathcal{L}(\mathbf{P}| \mathbf{I}, \mathbf{M})$, quantifying the discrepancy between the observed intraoperative image and the preoperative mesh $\mathbf{M}$ when positioned and oriented according to the pose $\mathbf{P}$.
%Given a preoperative surface mesh $M$ of the craniotomy area and an intraoperative image $I_{\text{intraop}}$ obtained from a surgical microscope, we seek to determine the pose $\hat{P}$ within the special Euclidean group $SE(3)$. This pose minimizes a loss function $\mathcal{L}$, quantifying the discrepancy between the observed intraoperative image and the preoperative mesh $M$ when positioned and oriented according to the pose $P$.
%The general formulation of the problem is shown in Eq. \ref{eq:general_problem}.
%\begin{equation}
%  \hat{P} = \underset{P \in SE(3)}{\mathrm{argmin}} \; \mathcal{L}(P| I_{\text{intraop}}, M)
%\label{eq:general_problem}
%\end{equation}

We approach the problem as an optimization in 2D image space. Our method minimizes the loss between $I$ and images rendered from a continuous and differentiable neural representation $f$ of the craniotomy area.
The density of $f$ is learned preoperatively from $M$ and its appearance is controlled intraoperatively by $I$. This approach effectively addresses the 3D-to-2D registration problem by using $f$ to render 2D images based on the anatomy learned from $M$. It also bridges the modality gap by incorporating intraoperative appearance conditioning on $I$.
We therefore reformulate the optimization problem with our neural representation $f$ and an image-based loss $\mathcal{L}_{rgb}$, yielding:
\begin{equation}
  \hat{\mathbf{P}} = \underset{\mathbf{P} \in SE(3)}{\mathrm{argmin}} \; \mathcal{L}_\text{rgb}(\mathbf{I}, f(\mathbf{P} | \mathbf{I}, \mathbf{M}))
\label{eq:image_problem}
\end{equation}

Given that $f$ is differentiable with respect to $\mathbf{P}$, we can find $\hat{\mathbf{P}}$ through iteratively rendering $f(\mathbf{P} | \mathbf{I}, \mathbf{M})$ and optimizing $\mathbf{P}$.

%Given that $f$ is differentiable with respect to $\mathbf{P}$, starting from an initialization $P_0$, we can find $\hat{P}$ through iteratively rendering $f(P | I, M)$ and optimizing $P$.

%Given that $F$ is differentiable back to $P$, we can initialize $P$ and iteratively render $F(P | I_{\text{intraop}}, M)$, compute $\frac{\partial \mathcal{L}}{\partial P}$, and update $P$, until $\hat{P}$ is found.

% \subsection{Building the Preoperative Training Dataset [1/2 page]}
% %\begin{itemize}
% %    \item We need to cross modalitieis, MRI to Camera images
% %    \item The synthesis function is critical
% %    \item Chose to rely on Neural Style Transfer
% %    \item Hybrid method, WCT+Strotts
% %    \item Sampling images from different viewpoints with different appearances
% %\end{itemize}

%\captionsetup[subfigure]{labelformat=empty}
%\begin{figure}[h!]
%\centering 
%\subfloat[Content (MR)]{\includegraphics[trim={4cm 4cm 4cm 6cm},clip, width=0.195\linewidth]{figs/NST/207_content.png}}
%\hfill
%\hfill
%\subfloat[WCT$^2$]{\includegraphics[trim={4cm 4cm 4cm 6cm},clip, width=0.195\linewidth]{figs/NST/207_207_wct_cat5.png}}
%\hfill
%\subfloat[STROTSS]{\includegraphics[trim={4cm 4cm 4cm 6cm},clip, width=0.195\linewidth]{figs/NST/207_207_strotss.png}}
%\hfill
%\subfloat[Ours (Hybrid)]{\includegraphics[trim={4cm 4cm 4cm 6cm},clip, width=0.195\linewidth]{figs/NST/207_207_cat5_1.0.png}}
%\hfill
%\subfloat[Style (Camera)]{\includegraphics[trim={4cm 4cm 4cm 6cm},clip, width=0.195\linewidth]{figs/NST/207_cam.png}} \\
%\hspace{-1.5em}
%\subfloat[Style 1]{\includegraphics[trim={0 0 0 4cm},clip, width=0.195\linewidth]{figs/NST/207_089_cat5_1.0.png}}
%\hfill
%\subfloat[Style 2]{\includegraphics[trim={0 0 0 4cm},clip, width=0.195\linewidth]{figs/NST/207_202_cat5_2.png}}
%\hfill
%\subfloat[Style 3]{\includegraphics[trim={0 0 0 4cm},clip, width=0.195\linewidth]{figs/NST/207_105_cat5_1.0.png}}
%\hfill
%\subfloat[Style 4]{\includegraphics[trim={0 0 0 4cm},clip, width=0.195\linewidth]{figs/NST/207_109_cat5_0.75.png}}
%\hfill
%\subfloat[Style 5]{\includegraphics[trim={0 0 0 4cm},clip, width=0.195\linewidth]{figs/NST/207_114_cat5_0.75.png}}
%\hfill
%\caption{-}
%\label{fig:res}
%\end{figure}

%\subsection{Single-Shot Style-Conditioned Neural Radiance Fields}
\subsection{Bridging the domain gap via Hypernetwork Multi-Style NeRF}
% \paragraph{\textbf{NeRF Background}}
% \begin{itemize}
%   \item Continous neural representation of scene
%   \item describing instant-ngp as this is what we are using
%   \item Consists of two major components, one for density (structure), one for RGB (appearance). Given a position $x$ and viewing direction $d$ yield density $\sigma(x)$ and color $c(x, d)$, the two components work in the following way:
%   \begin{itemize}
%     \item $\sigma(x), z(x) = F_{\text{density}}(x;\theta_{d}, \theta_{denc})$ where $\sigma(x)$ is the density, independent of viewing direction $d$, and $z(x)$ is as input to the second component
%     \item $c(x, d) = F_{\text{rgb}}(z(x), d;\theta_{rgb}, \theta_{rgbenc})$ where color $c$ is conditioned on output vector $z(x)$ of density function $F_{\text{density}}$ and viewing direction $d$.
%     \item Each component has learned input encodings and an MLP, therefore the two sets of parameters
%   \end{itemize}
%   \item TODO: mention other neural/implicit representations?
%   \item continuous neural representation can be used for rendering. Casting rays by evaluating NeRF along the way, collecting RGB values according to densities at each point
%   \item trained by supervising with a set of images of a scene, together with the camera poses for each image -> NeRF will try to reconstruct those images from the given poses and thereby learn the scene
%   \item Therefore, a continuous neural representation can be learned from a training set obtained from $M$.
%   \item Training set then by generating $N$ poses and images of $M$ textured with $t_{vr}$: $D = \{ (I_{1}, P_{1}), \ldots, (I_{N}, P_{N}) \}$
%   \item Serves our method as a neural rendering engine to represent our 3D mesh $M$ and enables us to render 2D images from any pose. Difference to mesh representation: fully differentiable and learnable, modifiable components. Both aspects key to our method, the former for iterative pose estimation, the latter to cross the domain gap to $I$. Explained in the following sections.
% \end{itemize}

\subsubsection{NeRF Background.}
A Neural Radiance Field (NeRF)~\cite{nerf} represents a continuous neural representation of a 3D scene. For our method, we follow Instant-NGP~\cite{instant_ngp}, a fast NeRF based on hash-grid encodings. The NeRF consists of a density (structure) and an RGB (appearance) component, evaluating a single point and viewing direction in space, is described mathematically by the following equations:
\begin{equation}
\sigma(\mathbf{x}), z(\mathbf{x}) = f_{\text{d}}(\mathbf{x}; \theta_{f_d}),
\label{eq:nerf1}
\end{equation}
where $\sigma(\mathbf{x})$ is the density and $z(\mathbf{x})$ is an intermediate representation used as input for the RGB component, and
\begin{equation}
c(\mathbf{x}, \mathbf{d}) = f_{\text{c}}(z(\mathbf{x}), \mathbf{d}; \theta_{f_c}),
\label{eq:nerf2}
\end{equation}
where the color $c$ depends on $z(\mathbf{x})$ and the viewing direction $d$. Both components consist of a Multilayer Perceptron (MLP), resulting in two sets of parameters, $\theta_{f_d}$ for density and $\theta_{f_c}$ for RGB. In practice, each component has a parametrized input encoding function, whose parameters are omitted here for clarity.

The continuous neural representation allows for rendering images by casting rays, evaluating the NeRF along each ray's path, and accumulating RGB values according to densities. For our method, NeRF serves as a neural renderer encoding our 3D mesh $\mathbf{M}$ (Fig. \ref{fig:overview}). This differs from traditional mesh representations since it is fully differentiable and has learnable disentangled components for structure $f_{d}$ and style $f_{c}$. Both aspects are key to our method, the former for iterative pose estimation, the latter to bridge the domain gap to $\mathbf{I}$.


% \paragraph{\textbf{Multi-style NeRF Background}}
% \begin{itemize}
%   \item high-level idea: two step process. First, train on whatever dataset (e.g. the one generated from $M$) to learn a preliminary NeRF.
%   \item will just learn the continuous representation of that scene. E.g., since $M$ is initially textured to have the appearance of the volume rendering of the preop scan (e.g. MRI), that NeRF will look indistinguishable from the volume-rendered brain surface in MR
%   \item second step: freeze the learned input encodings and most importantly, anatomy, encoded in the weights of the density MLP $\theta_{d}$
%   \item with the density and thereby structure of the NeRF fixed, learn style-dependent RGB networks to just change appearance of underlying anatomy
%   \item to do that: extending previous formulation of RGB network $F_{rgb}$ by conditioning the parameters of $\theta_{rgb}$ on a style $j$
%   % \item $c(x, d) = F_{\text{rgb}}(z(x), d; \theta_{\text{rgb}_j}, \theta_{rgbenc})$
%   \item goal of multi-style NeRF: given a single craniotomy image of any anatomy $I_{j}$, e.g. taken from a different craniotomy of another patient, modify $\theta_{rgb}$ and thereby the RGB MLP of the NeRF $F_{rgb}$ to render the learned anatomy of our mesh $M$ captured in $F_{dense}$ but with the appearance of $I_{j}$
%   \item How to learn those $\theta_{rgb_{j}}$? Keep NeRF training protocol, have one NeRF dataset for each style image $I_{j}$, use standard NeRF training procedure, everything but $\theta_{rgb_{j}}$ frozen because density is already learned -> learning individual RGB MLPs defined by $\theta_{rgb_{j}}$ for each $I_{j}$
%   \item The training set for each style defined by $I_{j}$ consists of $N$ images generated from the textured mesh $M$. Instead of applying the volume-rendering texture, we now create texture $t_j = NST(t_{vr}, I_j)$, where $NST(t_{vr}, I_j)$ denotes the style transfer from the original volume-rendering texture in MR appearance $t_{vr}$ to fit $I_j$
%   \item Training set then by generating $N$ poses and images of $M$ textured with $t_{j}$ instead of $t_{vr}$: $D_j = \{ (I_{j,1}, P_{j,1}), \ldots, (I_{j,N}, P_{j,N}) \}$
%   \item need for a figure to illustrate that $F_{\text{density}}$ learns from style transferred NeRF training set to find the pose of the untextured mesh $M$ in the WST dataset.
%   \item Why doing this? having multiple RGB nets while sharing one density net allows for a consistent anatomy across different possible intraoperative appearances of the brain surface, determining the "style" of $I$. Train $F_{\text{density}}$ on NeRF on arbitrary $D_i$ to ensure $F_{\text{rgb}}$ accuracy on multiple $D_i$.
% \end{itemize}


\subsubsection{Training the Hypernetwork Multi-Style NeRF.}
% \begin{itemize}
%   \item Having multiple RGB MLPs defined by $\theta_{j}$ that can be plugged into a NeRF representing one anatomy is beneficial, but since it is trained end-to-end as part of the entire NeRF, for every style $I_j$, we need $D_{j}$, which involves $NST$ to texture the $M$ and generate the $N$ training images and poses
%   \item Moreover, train RGB MLP from scratch
%   \item intraoperative setting: want to apply intraoperative appearance as observed in $I$ to our NeRF. But: not feasible to take microscope image $I_{intraop}$, run $NST$, create a training set, and learn $\theta_{rgb_{intraop}}$. Also, $NST$ gives most reliable results when guided with segmentation masks for vessels and parenchyma -> no problem preoperatively, but problem intraop
%   \item Therefore, we introduce a hypernetwork MLP $H$ that will \textit{predict} any $\theta_{rgb_{j}}$ from just a style image $I_{j}$
%   \item Thereby, first step: same as before for multi-style NeRF without hypernetwork, learning density
%   \item second step: instead of supervising NeRF training with different $D_{j}$ to learn individual $\theta_{rgb_{j}}$, we use the datasets to supervise another MLP $H$ to learn parameters $\phi$ such that $\theta_{rgb_{j}} = H(I_{j}; \phi)$
%   \item This leads to the following formulation of our NeRF. Note that this is formulation for the second step with the hypernetwork steering $F_{rgb_{j}}$. First step, "structure learning", follows standard NeRF formulation (ref equation X).
%   \item $\sigma(x), z(x) = F_{\text{density}}(x;\theta_{d}, \theta_{denc})$ where $\sigma(x)$ is the density, independent of viewing direction $d$, and $z(x)$ is as input to the appearance component.
%   \item $c(x, d) = F_{rgb_{j}}(z(x), d;H(I_{j};\phi), \theta_{rgbenc})$ where color $c$ is computed from an output vector $z(x)$ of density function $F_{\text{density}}$, viewing direction $d$. Note that $F_{rgb_{j}}$ has two sets of parameters: input encoding $\theta{rgbenc}$ learned during first step, and the parameters for the RGB MLP $\theta_{rgb_{j}} = H(I_{j};\phi)$
%   \item After training, we can tie $F_{rgb}$ and $F_{density}$ together with a ray casting technique that queries the two functions and their respective input encodings and MLPs. Our NeRF, formulated in a simplified manner, now forms a fully differentiable multi-style neural rendering engine $F$ that can render images $I_{render}$ from arbitrary camera poses $P$ for any given style image $I_{j}$:
%   \item $I_{render} = F(P, I_{j};H(I_{j};\phi))$
% \end{itemize}

%We train the NeRF model in two phases.
First, we train a NeRF following Eq.\ref{eq:nerf1} and Eq.\ref{eq:nerf2} on a dataset from the preoperative MR-derived surface mesh $\mathbf{M}$. 
%This dataset, textured to mimic the appearance of volume-rendered preoperative scans (e.g., MRI), serves to learn a continuous representation of the scene. 
The objective is to capture the anatomical structure with high fidelity, resulting in a NeRF that faithfully replicates the brain surface observed in MR scans.

We introduce a hypernetwork architecture that enables adapting to the intra-operative image appearance in real time using only one single image. 
The hypernetwork, that we denote $h$, takes the form of a multi-head MLP and is trained to set the parameters $\theta_{f_c}$ of $f_c$ based on the appearance of $\mathbf{I}$, leaving the structure, encoded in $f_{d}$, untouched.
To train $h$, we use Neural Style Transfer (NST) to stylize $\mathbf{M}$ from which we can generate NeRF training sets. 
We combine two NST approaches, WCT\textsuperscript{2}~\cite{wct2} for its strong preservation of semantic, and STROTSS~\cite{strotss} for a more photorealistic style.

%To learn multiple styles, we circle through a small dataset of style images $\mathbf{J}_i$ as input to $h$, and for each $\mathbf{J}_i$, we generate a style-specific training set $D_i$ to supervise the NeRF. 
%To generate $D_i$, we use the concatenation of two Neural Style Transfer (NST) methods, WCT\textsuperscript{2}~\cite{wct2} for its strong preservation of semantic, and STROTSS~\cite{strotss} for a more photorealistic style.
%We refer to the resulting style transfer method as CNST. Using CNST, For each $J_i$, we get a texture $t_i = \text{CNST}(t_{\text{VR}}, J_i)$ where $t_\text{VR}$ denotes the original volume-rendering texture. Then we apply $t_i$ to the mesh $M$, and render $N$ images from different poses to obtain $D_i$, a set of $N$ pairs of images and camera poses.



    
%The second phase uses a multi-head MLP hypernetwork $h$ to dynamically generate the parameters $\theta_{f_c}$ based on a given image $\mathbf{I}$. We refer to $I$, usually taken from a surgical microscope, as a style image because it controls ${f_c}$. To train $h$, all other parts of the NeRF are frozen after the first phase and the training protocol of ray casting and reconstructing training images for known camera poses does not change. 

This changes the NeRF formulation to the following.
\begin{equation}
    \sigma(\mathbf{x}), z(\mathbf{x}) = f_{d}(\mathbf{x}; \hat{\theta}_{f_d}),
\label{eq:density_hyper}
\end{equation}
\begin{equation}
    c(\mathbf{x}, \mathbf{d}) = f_{c}^{i}(z(\mathbf{x}), \mathbf{d}; h(J_i; \theta_h)),
\label{eq:rgb_hyper}
\end{equation}
where only $h$ is trained to learn $\theta_h$, while $\hat{\theta}_{f_d}$ has already been learned in the first phase.
In practice, $h$ uses a binned histogram of $J_i$ instead of the whole image, since the structural information is already provided by $f_{d}$, leading to relatively low-dimensional color-based features. All training is done preoperatively.



\subsection{Intraoperative Registration}
% \begin{itemize}
%     \item coming back to our problem formulation (ref equation X), can replace the rendering engine F with our method
%     \item $\hat{P} = \underset{P \in SE(3)}{\mathrm{argmin}} \; \mathcal{L}(I, F(P, I_{intraop};H(I_{intraop};\phi)))$
%     \item We leverage two properties of our NeRF $F$ to perform intraoperative registration. First, $H(I_{intraop};\phi)$ will set the parameters of the RGB MLP of $F$ to approximate $I_{intraop}$. Therefore, we can use a conventional RGB image loss to compare rendered images from $F$ to $I_{intraop}$. Second, since $F$ is a neural renderer and therefore fully differentiable, we can compute a gradient w.r.t to the input pose $P$ and update $P$.
%     \item Use existing method, slightly modified, that does this. Process: run $H(I_{intraop};\phi)$ to set weights of $F$. Pick initial pose $P$. Iterate until minimum and $\hat{P}$ is found: $I_{render} = F(P, I_{j};H(I_{j};\phi))$, compute loss between $I_{render}$ and $I_{intraop}$, update $P$.
%     \item practice, not rendering full images $I_{render}$ but just doing a collection of rays, does not matter for comparing with $I_{intraop}$ with pixel-wise loss
%     \item also, not using 1 init but many
%     \item Note that we assume camera intrinsics of surgical microscope and NeRF camera to be the same
% \end{itemize}
During surgery, we use $f_c$ and $f_d$ for a rendering engine $f$ that renders images via ray casting. Thus we can reformulate the initial optimization problem in Eq. \ref{eq:image_problem} as:

% \begin{equation}
%     I_{P,j} = F(P, I_{j}; \hat{\theta}_{d}, \hat{\theta}_{d\_enc}, \hat{\phi}, \hat{\theta}_{rgb\_enc})).
% \label{eq:rendering_engine}
% \end{equation}
\begin{equation}
    \hat{\mathbf{P}} = \underset{\mathbf{P} \in SE(3)}{\mathrm{argmin}} \; \mathcal{L}_{rgb}\big(\mathbf{I}, f(\mathbf{P}; \hat{\theta}_{f_d}, h(\mathbf{I}, \hat{\theta}_h))\big)  
\label{eq:problem_reformulated}
\end{equation}
% with
% \begin{equation}
%     %I_{P,intraop} = F(P; \hat{\theta}_{d}, \hat{\theta}_{d\_enc}, H(I_{intraop};\hat{\phi}), \hat{\theta}_{rgb\_enc})))
%     \hat{\mathbf{I}} = f(\mathbf{P}; \hat{\theta}_{d}, h(\mathbf{I}); \hat{\phi}), \hat{\theta}_{rgb})))
% \label{eq:I_render}
% \end{equation}

where $\mathbf{\hat{P}}$ represents the optimal camera pose, and $\mathcal{L}_{rgb}$ denotes the loss function comparing the intraoperative image $\mathbf{I}$ with images rendered by our method.

To solve registration tasks, we exploit two critical properties of $f$ for intraoperative registration. First, $h$ sets the style of $f$ through $\theta_{f_d} = h(\mathbf{I}; \hat{\theta}_{h})$. This allows us to express $\mathcal{L}_{rgb}$ as a conventional RGB image loss (relative $L_2$ loss \cite{parellel_inversion}) to evaluate the similarity between rendered and intraoperative images.

%\begin{equation}
%    \mathcal{L}(\text{prediction},\text{target}) = \frac{(\text{prediction} - \text{target})^2}{\left( \text{prediction}^2 + 0.01 \right)}
%\label{eq:relative_l2}
%\end{equation}

Second, the differentiable nature of $f$ allows computing $\frac{\partial \mathcal{L}}{\partial \mathbf{P}}$, thereby enabling iterative pose refinement via gradient descent. Multiple recent works explore inverting a NeRF in the described way. While iNeRF~\cite{inerf} follows the described approach closely, Parallel Inversion~\cite{parellel_inversion} achieves significantly better results in less time by computing $\frac{\partial \mathcal{L}}{\partial \mathbf{P}}$ on thousands of independent rays in parallel instead of reconstructing images first. PI-NeRF~\cite{pi_nerf} achieves comparable results to Parallel Inversion by using an additional invertible neural network that can estimate the pose without iterative optimization and an initial pose, making it two orders of magnitudes faster than Parallel Inversion and iNeRF. However, PI-NeRF has no publicly available codebase. Therefore, we choose Parallel Inversion with our style-conditioned neural rendering engine $f$ to solve Eq. \ref{eq:problem_reformulated} and estimate $\mathbf{\hat{P}}$. Note that an initial pose $\mathbf{P_{init}}$ is required and the optimization process is highly dependent on it. For neurosurgery, given extensive preoperative surgical planning, a rough camera pose of the surgical microscope is known and allows for sufficiently accurate initializations.



==> results-bis.tex <==
\section{Experiments and Results}

\subsubsection{Implementation Details}
% moving parts: our NeRF, instant ngp, parallel inversion, data generation
% TODO: come back to this: split of train and test set? runtime of training and parallel inversion? size of mlps? optimizer? how fast switching between hypernet datasets? how long initial training of hypernet? how long training in absolute time? normalization of styles that was used for real cases? 32 bins for histograms and concat of 3 channels to 96 features? cropping of targets? image sizes for hypernet and parallel inversion? masks that were used for style transfer? what about enhancement of the vrs?
% \begin{itemize}
%     \item for our NeRF: Nerfstudio (cite) environment, using their pytorch implementation of Instant-NGP
%     \item Parallel Inversion is only sota pose solver available but not in pytorch
%     \item in practice: rerender NeRF training set after hypernet inference, retrain NeRF in Parallel Inversion environment - also instant-ngp. No change in method, no perceivable change of quality.
%     \item style transfer methods also in pytorch
%     \item NeRF datasets from stylized textures are generated in pyvista
%     \item meshes $M$ and MR textures $tex_{vr}$ are done in 3D Slicer (cite)
%     \item slight modifications of Parallel Inversion: not using their second stage of resampling (no effect)
%     \item follow Parallel Inversion needs init, follow their way of evaluating; taking gt -> applying 15 degrees rot in all directions, applying small translation (relative to size of normalized scene), using that as init pose
%     \item TODO: mention difference in how we initialize this? for real cases: using exactly their values, 15 degree rot, 0.3 trans (but in their scale); for synthetic targets: 15 degrees rot, 5mm trans. Impossible to justify because just random
%     \item TODO: mention different rot range exploration? no one is going to understand
% \end{itemize}

Our style transfer, hypernetwork, and NeRF, following Instant-NGP, are built with Pytorch \cite{pytorch} and the Nerfstudio environment \cite{nerfstudio}. Parallel Inversion, however, is written in CUDA. Therefore, in practice, we rerender the NeRF training set post-hypernetwork inference and retrain in the Parallel Inversion environment. For pose estimation, we slightly modify Parallel Inversion, omitting the second stage of resampling, which we found to have no significant impact on results.

% TODO: mention different rot range exploration? no one is going to understand

% The generation of NeRF datasets from stylized textures is performed using PyVista, a Python tool for 3D visualization and analysis. The creation of meshes $M$ and their corresponding MR textures $tex_{vr}$ are conducted within the 3D Slicer platform, a software environment for medical image informatics.

% To initialize the pose estimation process, we adhere to the evaluation protocol established by Parallel Inversion. Ground truth poses are perturbed by applying a rotation of up to 15 degrees in all directions and a small translation, proportionate to the size of the normalized scene, to generate initial pose estimates.
% Our initialization process for real case scenarios precisely mirrors the parameters utilized by Parallel Inversion: a 15-degree rotation and a 0.3-unit translation in their normalized scale. For synthetic targets, we apply the same 15-degree rotation but adjust the translation to 5mm to accommodate the different scale.


\subsubsection{Datasets}
% \begin{itemize}
%     \item 15 style images
%     \item 4 clinical cases with MR and 1 surgical microscope image each
%     \item 1 additional case, MR but no surgical microscope image
%     \item 2 datasets, 1 for evaluation of clinical cases, 1 for evaluation on many synthetic surgical microscope images
%     \item clinical cases dataset: for each case!!!! create $M$ and $tex_{vr}$ from the craniotomy area of MR. 4 of the 15 style images correspond to the clinical cases -> leave out. For each of the other 11: generate texture via NST on initial $tex_{vr}$, then generate 100 random poses with textures $M$ -> 11 datasets of 100 images and camera poses each. Only 4 test images 
%     \item additional case dataset: Leaving out again the 4 real styles, generating and training with the other 11 datasets, that's identical to the other cases. However, since we only have 4 target poses in clinical cases, want to do more exhaustive evaluation on synthetic targets. For each of the 4 left out styles, instead of generating 100 images and poses for training, we generate 50 random images and poses as targets for pose estimation. Therefore: 11 styles with 100 images and poses each as training set, 4 styles with 50 images and poses each as test set. TODO: do I mention that we removed 1 of the 11 because of bad style transfer
% \end{itemize}

We test our method on 4 clinical cases, each with its MR and corresponding surgical microscope image, and an additional case with just an MR but no surgical microscope image. To stylize meshes, we rely on a small dataset of 15 surgical microscope images from different cases, including the 4 that correspond to our clinical test cases.
TODO: specify which ones are MRA/MRI T1/T2?

For the clinical cases, we built one dataset per case. We derived a 3D mesh $M$ and MR texture $tex_{vr}$ from the craniotomy area for each case. Then we applied NST with all 15 style images on the initial $tex_{vr}$. This yields 15 stylized meshes, for each of which we generate 100 images with their respective camera poses. For each case, this results in 1500 images that show the stylized brain surface mesh in 15 styles with 100 images and poses for each style. We generated data in the same way for the additional case. Additionally, for each of the 4 styles that correspond to the clinical cases, we generated 50 random images and poses as test targets for registration.

% TODO: this is not accurate, we trained those hypernets also on a 16th style 065, which we later excluded for the additional case because of bad NST. But mentioning 16 here and 15 there makes no sense?

\subsubsection{Synthesis}
To demonstrate that our hypernetwork produces plausible appearances, Fig. \ref{fig:synthesis} shows an example of $tex_{vr}$, the corresponding image $I$ from the surgical microscope, and synthesis results from several poses with our method. These results are obtained by training on the dataset for this case while omitting its style.

\captionsetup[subfigure]{labelformat=empty}
\begin{figure}[h!]
\subfloat{\includegraphics[width=0.245\linewidth]{figs/synthesis/mr_with_207.png}}
\hfill
\subfloat{\includegraphics[width=0.245\linewidth]{figs/synthesis/pose1.png}}
\hfill
\subfloat{\includegraphics[width=0.245\linewidth]{figs/synthesis/pose2.png}}
\hfill
\subfloat{\includegraphics[width=0.245\linewidth]{figs/synthesis/pose3.png}}\\
\caption{An example of synthesis from 3 different poses on one of the clinical cases. Left: Image obtained from volume rendering $tex_{vr}$ with surgical microscope image $I$. Rest: Synthesis with our rendering engine $F$, style inferred by hypernetwork $H$ on $I$.}
\label{fig:synthesis}
\end{figure}

\subsubsection{Pose Estimation on Synthetic Targets}
% \begin{itemize}
%     \item evaluating our method on additional case: 4 styles, 200 targets total
%     \item 4 styles -> for each, we infer style with hypernet once, then pose estimation for all 50 targets
%     \item showing accuracy-threshold curve for rotation and translation
%     \item showing relative number of predicted poses (y-axis) under threshold (x-axis) for all styles
%     \item outliers: pose estimation can diverge -> if rotation error > 20 degrees, we remove from evaluation and report as outlier
%     \item TODO: explain results with bad synthesis? how can I back this up? gram matrix tells nothing, pnsr tells nothing, only thing I can think of is histogram distribution?
% \end{itemize}
To evaluate our method on a larger number of registration targets, we use the additional case without surgical microscope image. Instead, we generated 50 targets for 4 different styles (corresponding to the clinical test cases), yielding 200 targets in total. The hypernetwork was trained on the remaining 11 styles. For each style, the hypernetwork conducts a singular inference to determine the style-specific appearance, which is then utilized in the pose estimation for all 50 targets within that style. The results are shown in accuracy-threshold curves (Fig. \ref{fig:acc_thres}), which indicate the proportion of predicted poses that fall within a given error threshold. %Outliers, defined as pose estimations with a rotation error greater than 20 degrees, are removed from the assessment and reported separately.

\captionsetup[subfigure]{labelformat=empty}
\begin{figure}[h!]
\subfloat[Style variance]{\includegraphics[width=0.20\linewidth]{figs/gram_scores_cross_correlation_matrix_clean.png}}
\hfill
\subfloat[Pose sampling]{\includegraphics[width=0.23\linewidth]{figs/pose_sampling2.png}}
\hfill
\subfloat[Rotations (deg)]{\includegraphics[width=0.27\linewidth]{figs/threshold_rot.png}}
\hfill
\subfloat[Translations (mm)]{\includegraphics[width=0.27\linewidth]{figs/threshold_trans_5mm.png}}
\hfill
\caption{Evaluation on synthetic targets (from left to right): pairwise Gram-Matrix of all styles showing pairwise style-similarity, pose distribution (blue: training, red: test), and accuracy-threshold curves for rotation and translation.}
\label{fig:acc_thres}
\end{figure}

As shown in Fig. \ref{fig:acc_thres}, rotation and translation errors vary depending on the style of the targets. While $96\%$ of poses estimated for Style 3 and Style 4 targets have a rotation error below 5°, it is $76\%$ and $54\%$ for targets of Style 2 and 1, respectively. Similarly, $96\%$ of poses estimated for Style 4 and $90\%$ of poses estimated for Style 3 have a translation error below 5mm, whereas the pose estimations on targets of Style 2 and 1 reach $78\%$ and $52\%$, respectively. We hypothesize that this is due to ...

TODO: explain results with bad synthesis? how can I back this up? gram matrix tells nothing, also tried pnsr (tells nothing), only thing I can think of is histogram distribution?
TODO: clean threshold curves from outliers? report outliers in text? probably makes more sense to leave outliers in for accuracy threshold curves? currently introducing outliers in the following section

%\begin{table}[ht]
%\centering
%\begin{tabular}{|l|c|c|c|c|}
%\hline
%Style & Style1 & Style2 & Style3 & Style4 \\ 
%\hline
%Avg Trans Error (mm) & 4.172 & 3.24 & 2.56 & 1.96 \\ 
%Avg Rot Error (deg)  & 4.53  & 3.25 & 2.41 & 1.84 \\ 
%Outliers (\%)        & 22    & 6    & 0    & 0    \\ 
%\hline
%\end{tabular}
%\caption{Registration Error for Different Styles}
%\label{tab:registration_error}
%\end{table}


\paragraph{\textbf{Comparison to Baseline and State-of-the-art}}


We evaluate our method against a baseline and the state-of-the-art. The baseline is our NeRF trained exclusively on images and poses from $M$ textured with $tex_{vr}$, which is visually equivalent to the volume rendering of the MR. The state-of-the-art pose estimation model for this task is a style-invariant regressor \cite{Haouchine2023}. Our method and the regressor are trained on the dataset of our additional case with 11 styles of 100 images and poses each, and evaluated on a test set of 4 styles of 50 images and ground-truth poses each. Given that most test poses differ from the training distribution (see red poses in \ref{fig:acc_thres}) which is inherently difficult for regression models, we also report results for the regressor when trained on 75\% of the original training set and evaluated only on the remainder of the training set (blue poses in \ref{fig:acc_thres}). We denote that as Reg. ID for "In Distribution". For all methods, we report the Average Translation Error (ATE), Average Rotation Error (ART). We also define outliers as poses with a rotation error larger than 20 degrees. Outliers are excluded from ATE and ART and reported separately as a percentage of the total amount of test poses. For our method, we additionally report results for all styles individually. Results are shown in Tab. \ref{tab:comparative_registration_error}.

\def\arraystretch{0.8}
\rowcolors{2}{}{gray!10}
\begin{table}[ht]
\centering
\caption{Comparative Registration Error}
\begin{tabular}{l|c|c|c|c!{\vline width 1.5pt}c|c|c|c}
\toprule
Metrics / Methods  &  \, Style1 \, & \, Style2 \, & \, Style3 \, & \, Style4 \, & \, \textbf{Ours} \, & \, MR \, & \, Reg. \, & \, Reg. ID \\ 
\midrule                    
Avg Trans. Er. (mm) & 4.17 & 3.24 & 2.56 & 1.96 & \textbf{3.12} & 10.12  &  13.31 & 6.29              \\ 
Avg Rot. Er (deg)  & 4.53  & 3.25 & 2.41 & 1.84 & \textbf{3.01} & 11.30  &  8.78 & 5.70               \\ 
Outliers (\%)        & 22    & 6    & 0    & 0 & 7   &  46.50   &  58 & 4.52  \\ 
\bottomrule
\end{tabular}
\label{tab:comparative_registration_error}
\end{table}

Our method outperforms both baseline and state-of-the-art and achieves average translation and rotation errors around 3mm and 3 degrees that meet clinical needs. However, we do not achieve style invariance with an increasing share of outliers for Style2 and Style1 compared to Style3 and Style4. Given that the underlying anatomy and target poses are the same across all styles, this indicates that the appearance approximated by our hypernetwork is not sufficiently similar enough to the target style to allow for a robust pose estimation with gradient descent. The MR-NeRF is not able to cross the modality gap to the target images and the regressor does not generalize to out-of-distribution target poses. Only when withholding and evaluating part of the more homogeneous training set does the performance of the regressor improve (Reg. ID in Tab. \ref{tab:comparative_registration_error}).

% \def\arraystretch{0.8}
% % \rowcolors{3}{}{gray!10}
% \begin{table*}[h!]
% \centering
% \caption{Validation on synthetic data and comparisons using real data.}
% \begin{tabular}{l | c | c | c | c | c | c | c | c | c }
% \toprule
%  & \multicolumn{3}{p{9em}|}{\centering Case 1} & \multicolumn{3}{p{9em}|}{\centering Case 2}  & \multicolumn{3}{p{9em}}{\centering Case 3} \\
%  \midrule
%  Method / Metric \hfill & TPR  \hfill  & FPR  \hfill  & MP \hfill  & TPR \hfill & FPR  \hfill  &  MP \hfill  & TPR \hfill  & FPR  \hfill  &  MP \hfill  \\
%  \midrule
%  SIFT \cite{x} + Cosine  &   4.77    &   95.22    &  153.7    &   2.91    &  97.08     &  182.5  &   2.09    &   97.90    & 224.03 \\
%  MIND \cite{x} + Cosine  &   1.65    &   98.34    &   200.0   &   0.88    &  99.11     &  200  &   0.88    &   99.11   & 200 \\  
%  SP \cite{x} + Cosine    &   4.58    &  95.41     &  150.8    &   2.76    &   97.23    &  144.83  &   3.82   &   96.17    &  147.58 \\  
%  SP + LG \cite{x}        &   55.31    &   44.68   &   25.28   &   13.06    &   86.93    &  13.60  &   17.99    &   82.00    &  16.34 \\  
%  Ours + LG   &    80.61   &   19.38    &  51.78    &   \textbf{76.92}    &   \textbf{23.07}    &  11.76  &    53.46   &   46.53   &  13.74 \\  
%  Ours + Cosine  &  \textbf{81.08}  &  \textbf{18.91}  &   50.14   &  73.42   &  26.57   &  44.64  &   \textbf{66.35}  &  \textbf{33.64}  & 53.96 \\  
%  \bottomrule
% \end{tabular}
% \label{tab:sota}
% \end{table*}


\paragraph{\textbf{Clinical Cases}}
% \begin{itemize}
%     \item for clinical cases -> no ground-truth
%     \item 6 DOF ground-truths highly subjective
%     \item show results qualitatively
%     \item works, but local minimum for one of the cases
% \end{itemize}
To evaluate each case, we exclude the style that belongs to that case and train our method on the remaining 14 styles with 100 images and poses each. Given that each case only has 1 corresponding surgical microscope image, we are limited to one pose estimation per case. Since we have no ground truth for our clinical cases and 6 DoF pose estimation is difficult with varying estimates between human annotators, we show qualitative results (Fig. \ref{fig:clinical}).

\captionsetup[subfigure]{labelformat=empty}
\begin{figure}[h!]
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/003/target_adjusted.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/003/step1.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/003/step2.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/003/registration.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/003/overlay.png}}\\
\hspace{-1.5em}
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/089/089_target_adjusted.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/089/step1.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/089/step2.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/089/registration.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/089/overlay.png}}\\
\hspace{-1.5em}
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/209/target_adjusted.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/209/step1.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/209/step2.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/209/registration.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/209/overlay.png}}\\
\hspace{-1.5em}
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/207/target_adjusted.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/207/step1.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/207/step2.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/207/registration.png}}
\hfill
\subfloat{\includegraphics[width=0.195\linewidth]{figs/clinical/paper_vis/207/overlay.png}}\\
\hspace{-1.5em}
\caption{Left column: intraoperative images of 4 clinical cases, obtained from surgical microscope. Middle columns: 3 steps of pose estimation with our method: first guess, mid-optimization, and final pose estimation. Right column: Intraoperative image with vessel-overlay of our estimated pose.}
\label{fig:clinical}
\end{figure}

\captionsetup[subfigure]{labelformat=empty}
\begin{figure}[h!]
\subfloat{\includegraphics[width=0.24\linewidth]{figs/bonus/089_mri_ori.png}}
\hfill
\subfloat{\includegraphics[width=0.24\linewidth]{figs/bonus/089_mri_ori.png}}
\hfill
\subfloat{\includegraphics[width=0.24\linewidth]{figs/bonus/089_tum2.png}}
\hfill
\subfloat{\includegraphics[width=0.24\linewidth]{figs/bonus/089_tum2.png}}
\caption{Tumor overlay and anatomy completion}
\label{fig:res}
\end{figure}

\section{Discussion \& Conclusion}
\begin{itemize}
    \item good qualitative results on clinical cases
    \item outperform sota on 200 synthetic targets
    \item in particular bad regressor and improved reg ID results support idea that continuous (neural) representation are a good way to cover the whole space of solutions
    \item hypernetwork not strong enough to make method style-invariant
    \item data-problem? only trained on 11 appearances
\end{itemize}
